The Effects of Peeling on Finite Element Method -based EEG Source Reconstruction

The problem of reconstructing brain activity from electric potential measurements performed on the surface of a human head is not an easy task: not just because the solution of the related inverse problem is fundamentally ill-posed (not unique), but because the methods utilized in constructing a synthetic forward solution themselves contain many inaccuracies. One of these is the fact that the usual method of modelling primary currents in the human head via dipoles brings about at least 2 modelling errors: one from the singularity introduced by the dipole, and one from placing such dipoles near conductivity discontinuities in the active brain layer boundaries. In this article we observe how the removal of possible source locations from the surfaces of active brain layers affects the localisation accuracy of two inverse methods, sLORETA and Dipole Scan, at different signal-to-noise ratios (SNR), when the H(div) source model is used. We also describe the finite element forward solver used to construct the synthetic EEG data, that was fed to the inverse methods as input, in addition to the meshes that were used as the domains of the forward and inverse solvers. Our results suggest that there is a slight general improvement in the localisation results, especially at lower noise levels. The applied inverse algorithm and brain compartment under observation also affect the accuracy.

==> set-pdf-version.tex <==
%%% set-pdf-version.tex
%
% This file is loaded by main.tex before any other operations, so that PDF
% version is set correctly for accessibility features.
%

\RequirePackage{luatex85}

\RequirePackage{ifluatex}

\def\mypdfminorversion{7}

\ifluatex

    \directlua {
        if pdf.getminorversion() \string~= \mypdfminorversion then
            if (status.pdf_gone and status.pdf_gone > 0)
            or (status.pdf_ptr and status.pdf_ptr > 0)
            then
                tex.error("PDF version cannot be changed anymore.")
            else
                pdf.setminorversion(\mypdfminorversion)
            end
        end
    }

    \pdfminorversion=\mypdfminorversion

\else

    \pdfminorversion=\mypdfminorversion

\fi

